Mitigating the BICM Loss in MIMO Receivers with Correlation-Informed Logits

Bit-interleaved coded modulation (BICM) is widely used in multiple-input multiple-output (MIMO) wireless systems. However, separating MIMO data detection from channel decoding and only exchanging per-bit soft information discards correlation information among the bits within each transmit vector. We show that the resulting information loss limits the performance of practical one-shot receivers. Even though iterative detection and decoding (IDD) can recover most of this loss, IDD significantly increases receiver complexity and latency. In order to reduce this loss, we propose COrrelation-Informed Logits (COIL), a soft-output format that combines per-bit soft information with pairwise coupling logits for correlated bits. We show how to incorporate these coupling logits into a conventional belief-propagation-based channel decoder, which enables correlation-aware decoding in a one-shot receiver without IDD. We evaluate COIL in a MIMO-BICM system with a conventional low-density parity-check code. For a 4x4 MIMO orthogonal frequency-division multiplexing (OFDM) system, a one-shot linear minimum mean-square error (LMMSE) receiver with COIL outperforms a conventional one-shot unbiased LMMSE receiver by 1.3dB and operates within 0.8dB of four-iteration IDD, while requiring only a single pass through the data detector.

==> sty/eth-colours.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% ETH Zürich's Corporate Design Colours
%%
%% Alexander Stutz (alstutz@iis.ee.ethz.ch)
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% corporate design colours
\definecolor{eth_blue}{RGB}{33, 92, 175}
\definecolor{eth_blue_10}{RGB}{233, 239, 247}
\definecolor{eth_blue_20}{RGB}{211, 222, 239}
\definecolor{eth_blue_60}{RGB}{122, 157, 207}
\definecolor{eth_blue_80}{RGB}{77, 125, 191}
\definecolor{eth_blue_120}{RGB}{8, 64, 126}

\definecolor{eth_petrol_120}{RGB}{0, 89, 109}
\definecolor{eth_petrol}{RGB}{0, 120, 148}
\definecolor{eth_petrol_10}{RGB}{231, 244, 247}
\definecolor{eth_petrol_20}{RGB}{204, 228, 234}

\definecolor{eth_green_120}{RGB}{60, 81, 30}
\definecolor{eth_green}{RGB}{98, 115, 19}
\definecolor{eth_green_10}{RGB}{239, 241, 231}
\definecolor{eth_green_20}{RGB}{224, 227, 208}
\definecolor{eth_green_60}{RGB}{161, 171, 113}
\definecolor{eth_green_80}{RGB}{129, 143, 66}
\definecolor{eth_green_120}{RGB}{54, 82, 19}

\definecolor{eth_bronze_120}{RGB}{107, 80, 31}
\definecolor{eth_bronze}{RGB}{142, 103, 19}
\definecolor{eth_bronze_10}{RGB}{244, 240, 231}

\definecolor{eth_red_120}{RGB}{150, 39, 45}
\definecolor{eth_red}{RGB}{183, 53, 45}
\definecolor{eth_red_80}{RGB}{197, 93, 87}
\definecolor{eth_red_10}{RGB}{248, 235, 234}
\definecolor{eth_red_20}{RGB}{241,215,213}

\definecolor{eth_purple_120}{RGB}{140, 10, 89}
\definecolor{eth_purple}{RGB}{167, 17, 122}
\definecolor{eth_purple_10}{RGB}{248, 232, 243}
\definecolor{eth_purple_20}{RGB}{239, 208, 227}

\definecolor{eth_grey_120}{RGB}{87, 87, 87}
\definecolor{eth_grey}{RGB}{111, 111, 111}
\definecolor{eth_grey_10}{RGB}{241, 241, 241}


% black and shades of grey
% (for non-white background check required opacity online)
\definecolor{eth_black}{RGB}{0, 0, 0}
\definecolor{eth_black_light}{RGB}{34, 34, 34}
\definecolor{eth_black_60}{RGB}{102, 102, 102}
\definecolor{eth_black_light_48}{RGB}{149,149,149}
\definecolor{eth_black_light_20}{RGB}{211, 211, 211}
\definecolor{eth_grey_10}{RGB}{241, 241, 241}
\definecolor{eth_grey_05}{RGB}{246, 246, 246}






==> sty/macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% Macros for the Paper 
%%
%% "Efficient and Physically-Consistent Modeling
%%  of Reconfigurable Electromagnetic Structures"
%%
%% Alexander Stutz, Georg Schwan, and Christoph Studer
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Color Palette:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{sty/eth-colours}

% corporate design colors
\colorlet{blue}{eth_blue}
\colorlet{blue_10}{eth_blue_10}
\colorlet{blue_20}{eth_blue_20}
\colorlet{blue_60}{eth_blue_60}
\colorlet{blue_80}{eth_blue_80}
\colorlet{blue_120}{eth_blue_120}

\colorlet{petrol_120}{eth_petrol_120}
\colorlet{petrol}{eth_petrol}
\colorlet{petrol_10}{eth_petrol_10}
\colorlet{petrol_20}{eth_petrol_20}

\colorlet{green_120}{eth_green_120}
\colorlet{green}{eth_green}
\colorlet{green_10}{eth_green_10}
\colorlet{green_60}{eth_green_60}
\colorlet{green_80}{eth_green_80}
\colorlet{green_120}{eth_green_120}

\colorlet{bronze_120}{eth_bronze_120}
\colorlet{bronze}{eth_bronze}
\colorlet{bronze_10}{eth_bronze_10}

\colorlet{red_120}{eth_red_120}
\colorlet{red}{eth_red}
\colorlet{red_80}{eth_red_80}
\colorlet{red_10}{eth_red_10}

\colorlet{purple_120}{eth_purple_120}
\colorlet{purple}{eth_purple}
\colorlet{purple_10}{eth_purple_10}
\colorlet{purple_20}{eth_purple_20}

\colorlet{black}{eth_black}
\colorlet{black_light}{eth_black_light}
\colorlet{black_60}{eth_black_60}
\colorlet{black_light_48}{eth_black_light_48}
\colorlet{black_light_20}{eth_black_light_20}
\colorlet{grey_120}{eth_grey_120}
\colorlet{grey}{eth_grey}
\colorlet{grey_10}{eth_grey_10}
\colorlet{grey_05}{eth_grey_05}

\definecolor{pink}{RGB}{214,82,130}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Tikz Macros:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pgfdeclarepatternformonly{south east lines my}{\pgfqpoint{-0pt}{-0pt}}{\pgfqpoint{5pt}{5pt}}{\pgfqpoint{5pt}{5pt}}{
    \pgfsetlinewidth{0.5pt}
    \pgfpathmoveto{\pgfqpoint{0pt}{5pt}}
    \pgfpathlineto{\pgfqpoint{5pt}{0pt}}
    \pgfpathmoveto{\pgfqpoint{.2pt}{-.2pt}}
    \pgfpathlineto{\pgfqpoint{-.2pt}{.2pt}}
    \pgfpathmoveto{\pgfqpoint{5.2pt}{4.8pt}}
    \pgfpathlineto{\pgfqpoint{4.8pt}{5.2pt}}
    \pgfusepath{stroke}}
    
\pgfdeclarepatternformonly{horizontal lines my}{\pgfqpoint{-0pt}{-0pt}}{\pgfqpoint{3.54pt}{3.54pt}}{\pgfqpoint{3.54pt}{3.54pt}}{
    \pgfsetlinewidth{0.5pt}
    \pgfpathmoveto{\pgfqpoint{0pt}{2pt}}
    \pgfpathlineto{\pgfqpoint{3.54pt}{2pt}}
    \pgfusepath{stroke}}

\pgfdeclarepatternformonly{diagonal behind text}{\pgfqpoint{-0pt}{-0pt}}{\pgfqpoint{15pt}{15pt}}{\pgfqpoint{15pt}{15pt}}{
    \pgfsetlinewidth{0.7pt}
    \pgfpathmoveto{\pgfqpoint{0pt}{0pt}}
    \pgfpathlineto{\pgfqpoint{15pt}{15pt}}
    \pgfpathmoveto{\pgfqpoint{14.8pt}{-.2pt}}
    \pgfpathlineto{\pgfqpoint{15.2pt}{.2pt}}
    \pgfpathmoveto{\pgfqpoint{-.2pt}{14.8pt}}
    \pgfpathlineto{\pgfqpoint{.2pt}{15.2pt}}
    \pgfusepath{stroke}}

\pgfdeclarepatternformonly{diagonal pattern node}{\pgfqpoint{-0pt}{-0pt}}{\pgfqpoint{3pt}{3pt}}{\pgfqpoint{3pt}{3pt}}{
    \pgfsetlinewidth{0.7pt}
    \pgfpathmoveto{\pgfqpoint{0pt}{0pt}}
    \pgfpathlineto{\pgfqpoint{3pt}{3pt}}
    \pgfpathmoveto{\pgfqpoint{2.8pt}{-.2pt}}
    \pgfpathlineto{\pgfqpoint{3.2pt}{.2pt}}
    \pgfpathmoveto{\pgfqpoint{-.2pt}{2.8pt}}
    \pgfpathlineto{\pgfqpoint{.2pt}{3.2pt}}
    \pgfusepath{stroke}}

\def\centerOfC at (#1,#2){
    \draw  [shift={(#1,#2)}, rotate=-45,line width=0pt, fill=white, color=white, anchor=center] (-.27,-.27) rectangle (.27,.27);
    \draw  [shift={(#1,#2)}, rotate=-45,line width=0pt, fill=white, color=white, anchor=center] (-.3,-.15) rectangle (.3,.15);

    
    \draw  [shift={(#1,#2)},line width=0.3pt, fill=white] (0,0) ellipse (0.16 and 0.16);
    \draw [shift={(#1,#2)},line width=0.3pt, color=black] (-0.2,0) -- (0.2,0);
    \draw [shift={(#1,#2)},line width=0.3pt, color=black] (0,-0.2) -- (0,0.2);
    \draw [shift={(#1,#2)},line width=0.3pt, color=black, fill=black]  (0,0) -- (0:0.16) arc (0:90:.16) -- cycle;
    \draw [shift={(#1,#2)},line width=0.3pt, color=black, fill=black]  (0,0) -- (180:0.16) arc (180:90+180:.16) -- cycle;
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Operators:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\DeclareMathOperator{\diag}{diag}			        % diag matrix
\DeclareMathOperator{\Ex}{\mathbb{E}}		        % expectation operator
\newcommand{\T}[0]{\mathsf{T}}                      % transpose
\newcommand{\He}[0]{\mathsf{H}}                     % hermitian
\DeclareMathOperator*{\argmax}{arg\,max}            % argmax
\DeclareMathOperator*{\maximize}{maximize}          % maximize               

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Font Macros:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\up}[1]{{\textnormal{#1}}}              % subscripts
\newcommand{\upc}[1]{{\textnormal{\textbf{#1}}}}    % subscripts in caption

\newcommand{\mat}[1]{{\bm{\mathbf{#1}}}}            % matrices
\newcommand{\vect}[1]{{\bm{\mathbf{#1}}}}           % vectors
\newcommand{\oper}[1]{\mathbb{#1}}                  % operator

\newcommand{\phs}[1]{{\color{pink}\mathsf{#1}}}  % phasor scalar
\newcommand{\phv}[1]{{\color{pink}\bm{\mathsf{#1}}}} % phasor vector


\newcommand*{\rom}[1]{\expandafter\@slowromancap\romannumeral #1@}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Fancy Ref Stuff
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand*{\fancyrefapplabelprefix}{app}		% Appendix
\newcommand*{\fancyrefthmlabelprefix}{thm}		% Theorem
\newcommand*{\fancyrefdefilabelprefix}{defi}    % Definition
\newcommand*{\fancyrefproplabelprefix}{prop}	% Proposition
\newcommand*{\fancyrefalglabelprefix}{alg}		% Algorithm
\newcommand*{\fancyrefasmlabelprefix}{asm}		% Assumption
\newcommand*{\fancyrefremlabelprefix}{rem}		% Remark
%\newcommand*{\fancyreftablabelprefix}{tab}		% Table


% label names
\frefformat{vario}{\fancyrefseclabelprefix}{Sec.~#1}
\frefformat{vario}{\fancyrefthmlabelprefix}{Thm.~#1}
\frefformat{vario}{\fancyrefdefilabelprefix}{Def.~#1}
\frefformat{vario}{\fancyreffiglabelprefix}{Fig.~#1}
\frefformat{vario}{\fancyrefapplabelprefix}{App.~#1}
\frefformat{vario}{\fancyrefeqlabelprefix}{(#1)}
\frefformat{vario}{\fancyrefproplabelprefix}{Prop.~#1}
\frefformat{vario}{\fancyrefalglabelprefix}{Alg.~#1}
\frefformat{vario}{\fancyrefasmlabelprefix}{Assu.~#1}
\frefformat{vario}{\fancyrefremlabelprefix}{Rem.~#1}
\frefformat{vario}{\fancyreftablabelprefix}{Table~#1}


\let\svthefootnote\thefootnote
\newcommand\blankfootnote[1]{%
  \let\thefootnote\relax\footnotetext{#1}%
  \let\thefootnote\svthefootnote%
}

%%%%% SPACE TWEAKS
%\linespread{0.980625} 
%\setlength{\textfloatsep}{10pt} % space under figure
%\setlength{\floatsep}{10pt} % space between two figure
%\setlength{\dbltextfloatsep}{10pt} % space under figure*
%\setlength{\dblfloatsep}{10pt} % space between two figure*

% vectors: boldface, no arrow (requested by CS)
\renewcommand{\vec}[1]{{\bm{\mathbf{#1}}}}

